Parts-Mamba: Augmenting Joint Context with Part-Level Scanning for Occluded Human Skeleton

Skeleton action recognition involves recognizing human action from human skeletons. The use of graph convolutional networks (GCNs) has driven major advances in this recognition task. In real-world scenarios, the captured skeletons are not always perfect or complete because of occlusions of parts of the human body or poor communication quality, leading to missing parts in skeletons or videos with missing frames. In the presence of such non-idealities, existing GCN models perform poorly due to missing local context. To address this limitation, we propose Parts-Mamba, a hybrid GCN-Mamba model designed to enhance the ability to capture and maintain contextual information from distant joints. The proposed Parts-Mamba model effectively captures part-specific information through its parts-specific scanning feature and preserves non-neighboring joint context via a parts-body fusion module. Our proposed model is evaluated on the NTU RGB+D 60 and NTU RGB+D 120 datasets under different occlusion settings, achieving up to 12.9% improvement in accuracy.

==> content/2_related_works.tex <==
\section{Related Works}

\subsection{State Space Model and Mamba}
\textbf{From S4 to Mamba.} Although self-attention has demonstrated its significant capability to capture dynamics within long sequences, its quadratic inference time complexity becomes a problem as the sequence length gets longer. Recently, State Space Models (SSM) have emerged as a compelling alternative for long sequence analysis other than self-attention-based structures, and the primary advantage of SSM lies in its dual sequential-parallel formulation, enabling linear inference complexity while being highly parallelizable during training. S4~\cite{gu2022efficiently} first introduced the HiPPO initialization for capturing long-range dependencies of language sequences with a kernel designed for achieving linear complexity during inference. S5~\cite{smith2023simplified} applied the parallel scan for all input dimensions to eliminate the channel mixing module in S4. H3~\cite{fu2023hungry} used two gated units along with S4 modules to formulate the self-attention-style query-key-value computation. GSS~\cite{mehta2023long} incorporated the gated unit for the S4 model to allow dimensionality reduction when performing the Fast Fourier Transform (FFT) operation. Then, Mamba~\cite{mamba} introduced the data-dependent structure with the selective parallel scan mechanism that can process long sequences as effectively as transformers while maintaining linear complexity.\\
\textbf{Mamba in Vision and Video Understanding.} Aside from the language domain, SSM also shows potential in other modalities. In the vision domain, Vim~\cite{vim} first introduced the Mamba-like bidirectional SSM structure for data-dependent visual modeling, achieving 2.8x faster inference speed than DeiT~\cite{deit}. In the video domain, Videomamba~\cite{videomamba} tried to extend the Mamba architecture into the video understanding domain with its proposed spatial-temporal scanning mechanism incorporated with the learnable spatial and temporal positional embeddings. It further introduces self-distillation into the Vim architecture.~\citet{videomamba2} further proposed the spatial-temporal reversal during the SSM scanning to improve the model's ability to model spatial-temporal relationships across patches.\\
\textbf{The Scanning Mechanism in Mamba.} One of the most important mechanisms inside the Mamba is its scanning mechanism. Because of the non-casual nature of the visual data, the default bidirectional scanning in Mamba results in a limited perceptive field. VMamba ~\cite{liu2024vmamba} proposed the 2D-Selective-Scan (SS2D) traversing spatial domain in four different directions and converting the image into a patch sequence to maintain the spatial structure and global relevance of the data. Efficient VMamba~\cite{pei2024efficientvmamba} applied an atrous selective scanning strategy to avoid redundant scanning and reduce the computations by sampling patches across the feature map.~\citet{yang_2024_3_plainmamba} utilized the continuous 2D scanning process to maintain the spatial adjacency of patches. LocalMamba~\cite{huang2024localmamba} divided the image patches into several non-interleaving windows and performed the selective scan inside each window to improve the model's ability to learn the localized feature representations.

Similar to the image patches, the non-casual nature also exists in skeleton joints since they are vectors with 3D positional information connected with a pre-defined adjacency that incorporates the body structure information. Inspired by the success of LocalMamba and VideoMamba, we proposed PartsMamba, which applied the parts-based scanning strategy to effectively enrich the local feature for the occluded scene in skeleton-based human action recognition.

\begin{figure*}[ht]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth]{figures/parts_mamba_main_blocks.pdf}}
    \caption{Overview of the proposed PartsMamba architecture.}
    \label{fig:parts_mamba_overview}
\end{figure*}

\subsection{Skeleton-Based Human Action Recognition and Occlusion}
RGB-based human action recognition is usually expensive and requires a large amount of computation, which makes it hard to deploy to devices like monitoring cameras or vision sensors for robots. To reduce the overall computations of action recognition~\cite{Johansson1973VisualPO} first utilized the 3D skeleton joint sequence to replace the original pixel input. As for now, skeleton-based action recognition has become one of the most popular and essential research topics in the computer vision domain. The current state-of-the-art model in skeleton-based human action recognition can be roughly divided into two main categories: GCN-only architecture and the hybrid GCN-Transformer architecture.\\
\textbf{The GCN-only Architecture.} In GCN-only architectures, ST-GCN~\cite{stgcn} first introduced the spatial-temporal graph convolution to make the model automatically learn both spatial and temporal joint feature patterns. After that, MS-G3D~\cite{MS-G3D} proposed a disentangled multi-scale aggregation scheme to remove redundant information and a unified spatial-temporal graph convolution to facilitate the spatial-temporal information flow. CTR-GCN~\cite{CTR-GCN} models the channel-wise topologies by adding a learnable shared topology as a generic prior for all channels. HD-GCN~\cite{HDGCN} applied a hierarchically decomposed graph to enable the GCN to thoroughly identify the significant distant edges between the same hierarchy node sets.\\
\textbf{The Hybrid Architecture.} Compared with GCNs, Transformers can easily capture the topology information inside the human skeleton and the relation of the non-connected joints, but their ability to capture local joint features and the joint dynamics in a short period is not powerful~\cite{ST-TR}. Therefore, the focus of recent works turned to the hybrid structure that uses GCN as an initial feature extraction module for aggregating the local and short-temporal features and a Transformer-based module as the context enhancer serving for long-distance joint relation and distant frame context extraction. Hyperformer~\cite{hyperformer} proposed a new self-attention mechanism on hypergraphs to help capture high-order relations inside the graph with the help of Multi-Scale Temporal Convolution (MS-TC) to model the temporal correlation of actions. Skeleton Mixformer~\cite{skeleton_mixformer} also used the multi-scale convolution with a temporal Transformer encoder to build its Temporal Mixformer part. \\
\textbf{The Occluded Scenario.} In real life, occlusion can frequently happen when the monitored human body parts are blocked by an obstacle (the spatial occlusion) or the bad frames are transmitted because of the poor signal (the temporal occlusion), and it is a challenging topic, while most of the models ignore the modeling robustness in the occluded scene. RA-GCN~\cite{RA-GCN} is the first paper addressing this challenge. It proposed a multi-stream GCN network that extracts different groups of joint representations and designed the experiment methodology of evaluating the model performance under the handcrafted occluded dataset. MSFGCN~\cite{MSFGCN} maintained that multi-stream structure and further designated the masked parts to augment the parts information in the human skeleton. PDGCN~\cite{PDGCN} proposed a dual inhibition training strategy to simulate the occlusion and use the Part-Aware Representation Learning (PARL) module to better extract spatial information. Other than making the end-to-end prediction, OP-GCN~\cite{OP-GCN} used an autoencoder-based occluded part detector to detect and reconstruct the missing parts and then feed them to the occlusion-aware GCN.

Our proposed PartsMamba model is a hybrid architecture with a GCN extracting local and short-term joint features and a spatial-temporal Mamba module capturing and refining both local and global correlations across joints.
